The Gaia Ultracool Dwarf Sample. I. Known L and T dwarfs and the first Gaia data release

We identify and investigate known ultracool stars and brown dwarfs that are being observed or indirectly constrained by the Gaia mission. These objects will be the core of the Gaia ultracool dwarf sample composed of all dwarfs later than M7 that Gaia will provide direct or indirect information on. We match known L and T dwarfs to the Gaia first data release, the Two Micron All Sky Survey and the Wide-field Infrared Survey Explorer AllWISE survey and examine the Gaia and infrared colours, along with proper motions, to improve spectral typing, identify outliers and find mismatches. There are 321 L and T dwarfs observed directly in the Gaia first data release, of which 10 are later than L7. This represents 45 % of all the known LT dwarfs with estimated Gaia G magnitudes brighter than 20.3 mag. We determine proper motions for the 321 objects from Gaia and the Two Micron All Sky Survey positions. Combining the Gaia and infrared magnitudes provides useful diagnostic diagrams for the determination of L and T dwarf physical parameters. We then search the Tycho-Gaia astrometric solution Gaia first data release subset to find any objects with common proper motions to known L and T dwarfs and a high probability of being related. We find 15 new candidate common proper motion systems.

==> table2.tex <==
    J0000+2554 &         2MASS 00001354+2554180 &    0.05643695 &   25.90501800 &              T4.5 & 2 &       6$\pm$ 19 &     130$\pm$ 22 &  15.063$\pm$0.039 & 1\\
    J0001+1535 &         2MASS 00011217+1535355 &    0.30074611 &   15.59319900 &                L4 & 2 &     150$\pm$ 19 &    -169$\pm$ 19 &  15.522$\pm$0.061 & 1\\
    J0001-0841 &         2MASS 00013166-0841234 &    0.38304167 &   -8.69080560 &        L1 p(blue) & 2 &     331$\pm$ 14 &    -299$\pm$ 14 &  15.712$\pm$0.049 & 1\\
    J0002+2454 &         2MASS 00025097+2454141 &    0.71239889 &   24.90393600 &              L5.5 & 2 &      10$\pm$ 28 &     -40$\pm$ 31 &  17.165$\pm$0.224 & 1\\
    J0004-6410 &         2MASS 00040288-6410358 &    1.01200620 &  -64.17661300 &          L1 gamma & 1 &      78$\pm$ 16 &     -55$\pm$ 36 &  15.786$\pm$0.071 & 1\\
    J0004-4044 &                      GJ 1001 B &    1.14519000 &  -40.73497000 &                L5 & 1 &     644$\pm$  3 &   -1494$\pm$  2 &  13.109$\pm$0.021 & 1\\
    J0005+3737 &       WISE J000517.48+373720.5 &    1.32291340 &   37.62233800 &                T9 & 2 &  -99999$\pm$*** &  -99999$\pm$*** &  18.330$\pm$0.120 & 2\\
    J0006+1540 &            ULAS J000613+154021 &    1.55416670 &   15.67250000 &                L9 & 2 &  -99999$\pm$*** &  -99999$\pm$*** & *******$\pm$***** & 0\\
    J0006-1720 &         2MASSI J0006205-172051 &    1.58545300 &  -17.34741200 &              L2.5 & 1 &     -32$\pm$ 17 &      17$\pm$ 18 &  15.662$\pm$0.064 & 1\\
    J0006-1319 &         2MASS 00062287-1319503 &    1.59445830 &  -13.33200000 &              L5 p & 2 &    -239$\pm$ 15 &    -413$\pm$ 18 &  16.674$\pm$0.125 & 1\\

